Induction by Coinduction and Control Operators in Call-by-Name

This paper studies emulation of induction by coinduction in a call-by-name language with control operators. Since it is known that call-by-name programming languages with control operators cannot have general initial algebras, interaction of induction and control operators is often restricted to effect-free functions. We show that some class of such restricted inductive types can be derived from full coinductive types by the power of control operators. As a typical example of our results, the type of natural numbers is represented by the type of streams. The underlying idea is a counterpart of the fact that some coinductive types can be expressed by inductive types in call-by-name pure language without side-effects.

==> eptcsdata.tex <==
\providecommand{\firstpage}{101}
\providecommand{\publicationstatus}{U. de'Liguoro and A. Saurin (Eds.):\\
Control Operators and their Semantics 2013 (COS'13)\\
EPTCS 127, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.127.7}{10.4204/EPTCS.127.7}}

